Bayesian reliability acceptance sampling plan with optional warranty under hybrid censoring

This work considers design of Bayesian reliability acceptance sampling plan (RASP) under hybrid censored life test for the products sold under optional warranty. The consumer and manufacturer agree on a common lifetime distribution of the product. However, they differ in the assessment of the prior distributions because of the adversarial nature of the consumer and manufacturer. The consumer takes decision based on his/her utility and prior belief without warranty offer by the manufacturer. If the decision is rejection, manufacturer provides warranty offer to the consumer. If the consumer rejects the lot with a warranty, the manufacturer conducts life test under hybrid censoring scheme (HCS) and provide lifetime information to the consumer. The consumer updates his/her belief based on lifetime information provided by the manufacturer. The consumer then takes decision of acceptance or rejection of lot based on updated belief. Task of the manufacturer is to determine the optimal life testing plan.

==> excess.tex <==
The manufacturer expected utility using (\ref{man}) we get 

\begin{align*}
\psi_M(m,\theta)= &[b_1{\theta^{q}}\Gamma(q+1)-b_2]I(c'(0)<nT_0)+\left[-c_a+\frac{c_a\theta}{w_2-w_1}\left[\exp(-w_1/\theta)-\exp(-w_2/\theta\right]\right]I(c'(0)<nT<c(0))\\
&\left.+b_3I(nT<c'(0))\right)\exp(-nT/\theta)+\sum_{d=1}^r[b_1{\theta^{q}}\Gamma(q+1)-b_2]P(TTT>c(d),D=d)\\
&+\sum_{d=1}^r\left[-c_a+\frac{c_a\theta}{w_2-w_1}\left[\exp(-w_1/\theta)-\exp(-w_2/\theta\right]\right]P(c'(d)<TTT<c(d),D=d)\\
&+\sum_{d=1}^rb_3P(TTT<c'(d),D=d)-b_4n-b_5E[D|\theta]-b_6E[\xi|\theta]
\end{align*}
\begin{table}[ht!]
\caption{Optimal design for different pre-fixed time points $T_0$ for the exponential distribution under RDSP approach.}
    \begin{center}
        \begin{tabular}
    {|ccccccc|}
       \hline  $T_0$& $\boldsymbol{m}^*=(n^*,r^*)$& $\psi_{\mathcal{M}}(\boldsymbol{m}^*)$&$(P(A_{wo}),P(A_{ww}),P(R))$ & $E[D]$&$E[\xi]$ & $L_w$\\
         \hline
     1&(5, 3)&80.91&(0.06, 0.76, 0.18) &0.45&0.99&2.37\\
      2&(6, 4) &83.85&(0.52, 0.36, 0.12)&1.02&1.98&1.06\\
      3&(4,3)&84.67&(0.51,0.36,0.13)&0.97&2.91&1.07\\
      4&(5,4)&84.64&(0.67, 0.23, 0.10)&1.48&3.91&0.65\\
      5&(3, 3)&85.01&(0.50, 0.37, 0.13)&1.08&4.84&1.08\\
      6&(3, 3)&84.67&(0.56, 0.31, 0.13)&1.21&5.73&0.91\\
      7&(3, 3)&84.52&(0.61, 0.26, 0.13)&1.33&6.58&0.76\\
      8&(3, 3)&84.36&(0.65, 0.23, 0.12)&1.44&7.41&0.65\\
       \hline
    \end{tabular}
    
    \end{center}

    \label{b12}
\end{table}
